Decomposing Overcomplete 3rd Order Tensors using Sum-of-Squares Algorithms

Tensor rank and low-rank tensor decompositions have many applications in learning and complexity theory. Most known algorithms use unfoldings of tensors and can only handle rank up to $n^{\lfloor p/2 \rfloor}$ for a $p$-th order tensor in $\mathbb{R}^{n^p}$. Previously no efficient algorithm can decompose 3rd order tensors when the rank is super-linear in the dimension. Using ideas from sum-of-squares hierarchy, we give the first quasi-polynomial time algorithm that can decompose a random 3rd order tensor decomposition when the rank is as large as $n^{3/2}/\textrm{polylog} n$. We also give a polynomial time algorithm for certifying the injective norm of random low rank tensors. Our tensor decomposition algorithm exploits the relationship between injective norm and the tensor components. The proof relies on interesting tools for decoupling random variables to prove better matrix concentration bounds, which can be useful in other settings.

==> omitproof__Tengyu_Ma_s_conflicted_copy_2015-04-17_.tex <==
\newpage

\section{Omitted Proofs in Section~\ref{sec:certify}}

\subsection{Proof of Lemma~\ref{lem:2-4norm}}\label{sec:2-4norm}
\label{sec:append:2to4}
We first restate the lemma here.

\begin{lemma}With high probability over the randomness of $a_i$'s, 
	\begin{equation}
	\sum_{i=1}^m \inner{a_i,x}^4\sosle_{r,12} 1+\widetilde{O}(m/n^{3/2}) \label{eqn:inter10}
	\end{equation}
\end{lemma}

%We are going to have an almost rigorous SoS proof. The slight non-rigorousness comes from the fact that we use some kind of recursive argument. 
%As in the $2\rightarrow 3$ norm case, we first use Chauchy-Shwarz to raise it into higher power: 

Recall \cite{BBH12} showed that when $m \ll n^2$, 

\begin{equation}
\sum_{i=1}^m \inner{a_i,x}^4\le O(1) \label{eqn:weak-2-4-norm}
\end{equation}

Here in order to improve this bound, we consider the square of the LHS of~\eqref{eqn:2-4norm} and apply Cauchy-Schwarz (similar to Claim~\ref{clm:cs}), 
\begin{align}
\left(\sum_{i=1}^m \inner{a_i,x}^4\right)^2 &= \left\langle\sum_{i=1}^m\inner{a_i,x}^3a_i, x\right\rangle^2\nonumber \\
&\sosle \left\|\sum_{i=1}^m\inner{a_i,x}^3a_i\right\|^2\|x\|^2 &\textrm{by Cauchy-Schwarz}\nonumber \\
&\sosle_r\left\|\sum_{i=1}^m\inner{a_i,x}^3a_i\right\|^2 = \sum_{i=1}^m \inner{a_i,x}^6 + \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^3\inner{a_j,x}^3\label{eqn:two-terms-2}
\end{align}

We will bound the first term of~\eqref{eqn:two-terms-2} by $1+o(1)$. We simply let $y = x^{\otimes 3}$ and let $B$ be the matrix whose $i$th row is $a_i^{\otimes 3}$. Then $f(y) = \|By\|^2$ has the property that $f(x^{\otimes 3}) =  \sum_{i=1}^m \inner{a_i,x}^6$. Therefore it suffices to prove that $f(y)\sosle (1 + o(1)\|y\|^2$ or equivalently $\|B\|\le 1+o(1)$. %Then we can rewrite 

%$$\sum_{i=1}^m \inner{a_i,x}^6 = \|By\|^2$$

Consider the matrix $BB^T$. It is a $n$ by $n$ matrix with diagonal entries 1 and off diagonal entries of the form $\inner{a_i^{\otimes 3},a_j^{\otimes 3}} = \inner{a_i,a_j}^3$. 
By the incoherence of $a_i$'s, we have $\inner{a_i,a_j}^3 \lesssim 1/n^{3/2}$. Then by Gershgorin disk theorem, we have $\|BB^T\|\le 1+\widetilde{O}(m/n^{3/2})  = 1+\delta$. It follows that $\|B\|\le 1+\widetilde{O}(m/n^{3/2})$.  Therefore, 
\begin{equation}
\sum_{i=1}^m \inner{a_i,x}^6 = \|Bx^{\otimes 3}\|^2 \sosle (1+\widetilde{O}(m/n^{3/2}))\|x^{\otimes 3}\| \le_r 1+\widetilde{O}(m/n^{3/2}) \label{eqn:inter6}
\end{equation}

For the second term of~\eqref{eqn:two-terms-2}, we apply Cauchy-Schwarz again: 

\begin{align}
\left(\sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^3\inner{a_j,x}^3\right)^2 &\sosle   \left(\sum_{i\neq j}\inner{a_i,a_j}^2\inner{a_i,x}^2\inner{a_j,x}^2\right) \left(\sum_{i\neq j}\inner{a_i,x}^4\inner{a_j,x}^4\right) \nonumber\\
&\sosle \left(\frac{1}{n}\cdot \sum_{i}\inner{a_i,x}^2\sum_j \inner{a_j,x}^2\right) \left(\sum_{i}\inner{a_i,x}^4\sum_j \inner{a_j,x}^4\right) \label{eqn:inter4}
\end{align}

Note that the matrix $A =[a_1\vert \dots\vert a_m]$ has spectral norm bound  $\|A\|\lesssim \sqrt{m/n}$, and therefore 
$$\sum_{i}\inner{a_i,x}^2 = \|A^Tx\|^2 \sosle \|A\|^2 \|x\|^2 \sosle_r \|A\|^2$$
Then using Equation~\ref{eqn:weak-2-4-norm}, and the equation above, we have %the spectral norm of $[a_1\vert \dots\vert a_m]$, we have 
\begin{align}
%\left(\sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^3\inner{a_j,x}^3\right)^2 
%&\le \left(\frac{1}{n}\cdot \sum_{i}\inner{a_i,x}^2\sum_j \inner{a_j,x}^2\right) \left(\sum_{i}\inner{a_i,x}^4\sum_j \inner{a_j,x}^4\right)\\
\textrm{RHS of~\eqref{eqn:inter4} }& \sosle_r \frac{1}{n}\cdot \frac{m}{n} \cdot \frac{m}{n} \cdot O(1) \cdot O(1) \le \widetilde{O}(m^2/n^3) \label{eqn:inter5}
\end{align}

Then by ~\ref{eqn:inter4} and ~\ref{eqn:inter5} and Lemma~\ref{lem:square-root}, we have that 
\begin{equation}
\sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^3\inner{a_j,x}^3 \sosle_r \widetilde{O}(m^2/n^3) \label{eqn:inter7}
\end{equation}

Hence, combining equation~\eqref{eqn:inter7}, ~\eqref{eqn:inter6} and~\eqref{eqn:two-terms-2} we have that 



\begin{align}
\left(\sum_{i=1}^m \inner{a_i,x}^4\right)^2 
&\sosle_r \sum_{i=1}^m \inner{a_i,x}^6 + \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^3\inner{a_j,x}^3\nonumber\\
& \sosle_r 1+ \widetilde{O}(m/n^{3/2})  + \widetilde{O}(m/n^{3/2})   = 1+\widetilde{O}(m/n^{3/2}) \label{eqn:inter11}
\end{align}
Using Lemma~\ref{lem:square-root} again, we complete the proof of Lemma~\ref{eqn:2-4norm}. 
%\begin{remark}
%	In principle, we don't even have to use the result of ~\cite{DBLP:journals/corr/abs-1205-4484} at all. But then we have a recursive SoS proof, which should also be doable but a little bit messy. 
%\end{remark}



%\subsection{Bounding $p(x)$}\label{sec:px}
%
%Recall $p(x) = \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i,x}^2\inner{a_j,x}^2$ is a degree-4 polynomial of $x$. The general idea is simply to let $y= x^{\otimes 2}$ and write $p(x)$ as a degree-2 polynomial of $y$, and then apply random matrix theory. However, instead of doing the naive way that we write $p(x) = \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i^{\otimes 2},x^{\otimes 2}}\inner{a_j^{\otimes 2}, x^{\otimes 2}}$, and replace $x^{\otimes 2}$ by $y$, we take a slightly different approach. Note that 
%
%$$p(x) = \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i\otimes a_j,x^{\otimes 2}}\inner{a_i\otimes a_j, x^{\otimes 2}}$$
%
%It suffices to prove that via SoS (modulo $\|y\|^2 = 1$)
%
%$$ \sum_{i\neq j}\inner{a_i,a_j}\inner{a_i\otimes a_j,y}\inner{a_i\otimes a_j, y} \le 1+o(1)$$
%
%We can write this as a quadratic form $y^TMy$ using a $n^2\times n^2$ matrix $M$ defined as 
%
%$$M        = \sum_{i\neq j}\inner{a_i,a_j} (a_i\otimes a_j) (a_i\otimes a_j)^T $$
%
%%To bound the spectral norm of $M$, we further rewrite $M$. Let $A = [a_1\vert a_2 \dots \vert a_m]$ and let $B: =A\otimes A$ be the Kronecker product of $A$ and $A$. (Therefore $B$ is a $n^2\times m^2$ matrix, and one can verify that the $(i,j)$-th column of $B$ is indeed $a_i\otimes a_j$. ) Let $b$ be the $m^2$ dimensional vector whose $(i,j)$-th entry is $\inner{a_i,a_j}$ if $i\neq j$, and 0 otherwise.  Then we can rewrite $M$ as 
%
%%\begin{equation}
%%M = B\diag(b)B^T \label{eqn:form-M}
%%\end{equation}
%
%
%We claim that $M$ has spectral norm at most $o(1)$ with whp. 
%
%\begin{lemma}\label{claim:spectral_bound}when $m \ge n$ and $m\ll n^{3/2}$, we have 
%$$\|M\|\le \widetilde{O}(m/n^{3/2})$$
%
%\end{lemma}

\subsection{Proof of Lemma~\ref{lem:px}}\label{sec:px}

We first restate the lemma:

\begin{lemma}\label{lem:restate-px}
When $m\ll n^{3/2}$, the matrix $M = \sum_{i\neq j}\inner{a_i,a_j} (a_i\otimes a_j) (a_i\otimes a_j)^T$ has spectral norm at most $\widetilde{O}(m/n^{3/2})$ and as a direct consequence, 
$$p(x)\sosle_{r,4} \widetilde{O}(m/n^{3/2})$$
\end{lemma}


\begin{proof}
As suggested in the proof sketch, we first use a simple symmetrization which allows us to focus on the randomness of signs of $\inner{a_i,a_j}$.  For simplicity of notation, let $Q_{ij} := \inner{a_i,a_j}(a_i\otimes a_j) (a_i\otimes a_j)^T$.  Let $\sigma\in \{\pm 1\}^m$ be uniform random $\pm 1$ vector and define $M'$ as 
	$$M' =  \sum_{i\neq j} \sigma_i\sigma_jQ_{ij}.$$
	We claim that $M'$ has the same distribution as $M$, since $a_i$ has the same distribution as $\sigma_ia_i$. Then from now on we condition on the event that $a_i$'s have incoherence property and low spectral norm, that is, $\inner{a_i,a_j}\lesssim 1/\sqrt{n}$,   $\|A\| = \left\|[a_1\vert a_2 \dots \vert a_m]\right\|\lesssim \sqrt{m/n}$, and we will only focus on the randomness of $\sigma$. Ideally we want to write $M'$ as a sum of independent random matrices so that we can apply matrix Bernstein inequality. However, now the random coefficients are $\sigma_i\sigma_j$, and they are not independent with each other.
	
	A key observation here is that the sum is only over the indices $(i,j)$ with $i\neq j$, therefore we can use Theorem 1 of~\cite{decoupling} (restated as Theorem~\ref{thm:decoupling} in the end) to decouple the correlation first. 
	
	Theorem~\ref*{thm:decoupling} basically says that to study the concentration of  a sum of the form $\sum_{i\neq j}f_{ij}(X_i,X_j)$, it is up to constant factor similar to the concentration of the sum $\sum_{i\neq j}f_{ij}(X_i,Y_j)$ where $Y_i$ is an independent copy of $X_i$. Applying the theorem to our situation, we have that there exists absolute constant $C$ such that 
	\begin{equation}
	\Pr[\|M'\|\ge t] \le C\Pr[M''\ge t/C] \label{eqn:M'-M''}
	\end{equation}
	where $$M'':= \sum_{i\neq j}\sigma_i\tau_jQ_{ij},$$ and $\sigma,\tau$ are independently uniform over $\{-1,+1\}^m$. 
	
	 %(and they are independent of each other as well).
	Now it suffices to bound the norm of $M''$. We proceed by rewriting $M''$ as 
	$$M'' = \sum_i {\sigma_i \sum_{j\neq i}\tau_jQ_{ij}} := \sum_i \sigma_i T_i,$$
	where \begin{equation}
	T_i :=  \sum_{j\neq i}\tau_jQ_{ij} \label{eqn:T_i}
	\end{equation}
	
	We study the properties of $T_i$ first. 
	
\begin{claim}\label{claim:T}
With high probability over the randomness of $a_i$'s, for all $i$, $T_i \preceq \tilde{O}(\sqrt{m}/n) (a_i a_i^T) \otimes I$.
\end{claim}
	
\begin{proof}	
	
	Recall that $Q_{ij} =  \inner{a_i,a_j}(a_i\otimes a_j) (a_i\otimes a_j^T)$. In the definition~\ref{eqn:T_i} of $T_i$, the index $i$ is fixed and we take sum over $j$. Therefore it will be convenient to write $Q_{ij}$ as $Q_{ij} = \inner{a_i,a_j}(a_ia_i^T)\otimes (a_ja_j)^T$ where $\otimes$ is the Kronecker product between matrices. Then $T_i$ can be written as 
	
	$$T_i = (a_ia_i^T)\otimes \left(\sum_j\tau_j\inner{a_i,a_j}a_ja_j^T\right).$$
	
	We apply the Bernstein inequality on the right factor. Matrix Bernstein bound requires spectral norm bound for individual matrices, and a variance bound.
	
For the spectral norm of individual matrices, we check that $ \|\tau_j\inner{a_i,a_j}a_ja_j^T\|\lesssim 1/\sqrt{n}$ (by incoherence).
For variance we know $$\|\Exp[\sum_{j}\tau_j^2(\inner{a_i,a_j}a_ja_j^T)^2]\| = \|A\diag(\inner{a_i,a_j}^2)_{j\neq i}A^T\|\lesssim m/n^{2},$$ 
where we used the spectral norm of $A$ and the fact that $\inner{a_i,a_j}^2 \lesssim 1/n$.

Therefore by Matrix Bernstein's inequality we have that  whp, over the randomness of $\tau$, 
	$$\|\sum_j\tau_j\inner{a_i,a_j}a_ja_j^T\| \le \widetilde{O}(\sqrt{m}/n).$$
	
Using the fact that for two matrices $P$ and $Q$, if $P\preceq Q$ and $R$ is PSD, then $R\otimes P\preceq R\otimes Q$ (see Lemma~\ref{lem:psdkronecker}),  it follows that 
	$$T_i \preceq (a_ia_i^T)\otimes (\widetilde{O}(\sqrt{m}/n)\cdot I).$$

Finally we use union bound and conclude with high probability this is true for any $i$.
\end{proof}

%	Then we have $$M''  = \sum_i \sigma_i T_i \le \left(\sum_i \sigma_i a_ia_i^T\right)\otimes (\sqrt{m}/n\cdot I)$$

Now we can apply matrix Bernstein for the sum $M'' = \sum_{i=1}^m \sigma_i T_i$. The individual spectral norm is bounded by $\tilde{O}(\sqrt{m}/n)$ by the Claim~\ref{claim:T}. The variance is
$$
\|\sum_{i=1}^m T_i^2\| \le \tilde{O}(m/n^2)\|\sum_{i=1}^m ((a_ia_i^T)\otimes I)^2\|
= \tilde{O}(m/n^2)\|(AA^T)\otimes I\| = \tilde{O}(m^2/n^3).
$$

	Using matrix Bernstein inequality, we know with high probability $\|M''\| \le \tilde{O}(m/n^{3/2})$.
	
	Using (\ref{eqn:M'-M''}), we get that whp, $\|M'\|\le \widetilde{O}(m/n^{3/2})$. Since $M'$ and $M$ has the same distribution, we conclude that  whp, $\|M\|\le \widetilde{O}(m/n^{3/2})$. 
	
\end{proof}

\subsection{Main Theorem for Certifying Injective Norm}
\label{sec:append:certifymain}
Now we are ready to prove Theorem~\ref{thm:maininjdet}.

\begin{theorem}
Algorithm~\ref{alg:certifying-norm}  always returns NO when $\|T\|_{\textrm{inj}} > 1+1/\log n$. When $T\sim \mathcal{D}_{m,n}$ and $m\ll n^{3/2}$, Algorithm~\ref{alg:certifying-norm} returns YES with high probability over the randomness of $T$. Further, the same guarantee holds given an approximation $\tilde{T}$ where if $M \in \R^{n\times n^2}$ is an unfolding of $T - \tilde{T}$, $\|M\| \le 1/2\log n$. 
\end{theorem}

\begin{proof}
We first prove whenever $\|T\|_{\textrm{inj}} > 1+1/\log n$, the algorithm returns NO. This is because a large injective norm implies there exists an unit vector $x^*$ with $T(x^*,x^*,x^*) = 1$. We can construct a pseudo-expectation $\pE$ as $\pE[p(x)] = p(x^*)$. Clearly this is a valid pseudo-expectation (it is even the expectation of a true distribution: $x = x^*$ with probability 1). Also, we know $\pE[T(x,x,x)] = T(x^*,x^*,x^*) > 1+1/\log n$, so in particular $OPT > 1+1/\log n$ and the algorithm must return NO.

Next we show the algorithm returns YES with high probability when $T$ is chosen from $\mathcal{D}$. This follows directly from Theorem~\ref{thm:proof}, which in turn follows from Lemmas~\ref{lem:2-4norm} and \ref{lem:px}. In particular, we know there is a degree-12 SoS proof that shows $T(x,x,x) \le 1+\tilde{O}(m/n^{3/2}) \le 1+1/2\log n$, so by Lemma~\ref{lem:sos} this must also hold for any pseudo-expectation.

When we are only given tensor $\tilde{T}$ such that the unfolding of $\tilde{T}-T$ has spectral norm $1/2\log n$. Let $M$ be the unfolding of $\tilde{T}-T$, and $y = x\otimes x$, then by Lemma~?? we know $(x^TMy)^2 \preceq \|x\|^2 \|M\|^2 \|y\|^2$, which implies (by Lemma~\ref{}) $[\tilde{T}-T](x,x,x) = x^TMy \sosle_{r,12} \|M\| \le 1/2\log n$. Combining the two terms we know
$$
\tilde{T}(x,x,x) = T(x,x,x)+[\tilde{T}-T](x,x,x) \sosle_{r,12} 1+1/\log n.
$$
\end{proof}

\input{omitproof2}



